The Chow--Witt rings of the classifying space of quadratically oriented bundles

In this paper we compute the Chow--Witt rings of the classifying space ${\rm BSL}_n^c$ of quadratically oriented vector bundles of rank $n$. We also discuss the corresponding quadratically-oriented cobordism spectrum ${\rm MSL}^c$ and show that it is equivalent to $\rm{MSL}$ after inverting $\eta$.

==> commands.tex <==
% Packages
\RequirePackage{amsmath,amssymb,amsthm,thmtools}
\RequirePackage{amsfonts}
\RequirePackage{geometry}
\RequirePackage{color}
\RequirePackage{mathtools}
\RequirePackage{bbm}
\RequirePackage{mathrsfs}
\RequirePackage{tikz}
\usepackage[shortlabels]{enumitem}
\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{cd}
\tikzstyle{arrow} = [thick,->,>=stealth]

% Arrows
\providecommand{\po}{\arrow[ul,phantom,"\ulcorner" very near start]}
\providecommand{\pb}{\arrow[dr,phantom,"\lrcorner" very near start]}
\providecommand{\xto}[1]{\xrightarrow{#1}}
\providecommand{\from}{\leftarrow}
\providecommand{\xfrom}[1]{\overset{#1}{\leftarrow}}

\providecommand{\mapsfrom}{\mathrel{\reflectbox{\ensuremath{\mapsto}}}}
\providecommand{\longmapsfrom}{\mathrel{\reflectbox{\ensuremath{\longmapsto}}}}

\providecommand{\hookto}{\xhookrightarrow{}}
\providecommand{\xhookto}[1]{\overset{#1}{\hookrightarrow}}

\providecommand{\hookfrom}{\xhookleftarrow{}}
\providecommand{\xhookfrom}[1]{\xhookleftarrow{#1}}

\providecommand{\tto}{\twoheadrightarrow}
\providecommand{\xtto}[1]{\overset{#1}{\twoheadrightarrow}}
\providecommand{\ffrom}{\twoheadleftarrow}
\providecommand{\xffrom}[1]{\overset{#1}{\ffrom}}

\providecommand{\ladjoint}[2]{ #1\rightleftarrows #2 }
\makeatletter
\providecommand{\superimpose}[2]{%
  {\ooalign{$#1\@firstoftwo#2$\cr\hfil$#1\@secondoftwo#2$\hfil\cr}}}
\makeatother
\providecommand{\smallslash}{\mbox{\tiny/}}

\providecommand{\clhookto}{\mathrel{\raisebox{0.1em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.1em}\smallslash}{\hookrightarrow}}}$}}}
\providecommand{\xclhook}[1]{\overset{#1}{\clhook}}

\providecommand{\clhookfrom}{\mathrel{\raisebox{0.1em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.1em}\smallslash}{\hookleftarrow}}}$}}}

\providecommand{\ohookto}{\mathrel{\raisebox{0.03em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.03em}\mbox{\small$\circ$}}{\hookrightarrow}}}$}}}

\providecommand{\ohookfrom}{\mathrel{\raisebox{0.03em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.03em}\mbox{\small$\circ$}}{\hookleftarrow}}}$}}}

\providecommand{\cofto}{\rightarrowtail}
\providecommand{\coffrom}{\leftarrowtail}
\providecommand{\xcofto}[1]{\overset{#1}{\cofto}}
\providecommand{\xcoffrom}[1]{\overset{#1}{\coffrom}}

% Common Text Commands
\providecommand{\ab}{\text{ab}}
\providecommand{\ann}{\text{ann}}
\providecommand{\Aut}{\text{Aut}}
\providecommand{\BSL}{\text{BSL}}
\providecommand{\char}{\text{char}}
\providecommand{\cl}{\text{cl}}
\providecommand{\codim}{\text{codim}}
\providecommand{\coev}{\text{coev}}
\providecommand{\colim}{\text{colim}}
\providecommand{\conj}{\text{conj}}
\providecommand{\const}{\text{const}}
\providecommand{\Disc}{\text{Disc}}
\providecommand{\End}{\text{End}}
\providecommand{\EKL}{\text{EKL}}
\providecommand{\ev}{\text{ev}}
\providecommand{\Fix}{\text{Fix}}
\providecommand{\Frac}{\text{Frac}}
\providecommand{\Frob}{\text{Frob}}
\providecommand{\Fun}{\text{Fun}}
\providecommand{\Gal}{\text{Gal}}
\providecommand{\GL}{\text{GL}}
\providecommand{\gr}{\text{gr}}
\newcommand{\GW}{\text{GW}}
\providecommand{\Hom}{\text{Hom}}
\providecommand{\id}{\text{id}}
\providecommand{\im}{\text{im}}
\renewcommand{\Im}{\text{Im}}
\providecommand{\incl}{\text{incl}}
\providecommand{\Ind}{\text{Ind}}
\providecommand{\Inn}{\text{Inn}}
\providecommand{\Jac}{\text{Jac}}
\providecommand{\Map}{\text{Map}}
\providecommand{\mult}{\text{mult}}
\providecommand{\op}{\text{op}}
\providecommand{\Orb}{\text{Orb}}
\providecommand{\ord}{\text{ord}}
\providecommand{\Out}{\text{Out}}
\providecommand{\Perm}{\text{Perm}}
\providecommand{\pr}{\text{pr}}
\providecommand{\pre}{\text{pre}}
\providecommand{\PSL}{\text{PSL}}
\providecommand{\quot}{\text{quot}}
\providecommand{\rank}{\text{rank}}
\renewcommand{\Re}{\text{Re}}
\providecommand{\Res}{\text{Res}}
\providecommand{\sgn}{\text{sgn}}
\providecommand{\sig}{\text{sig}}
\providecommand{\SL}{\text{SL}}
\providecommand{\soc}{\text{soc}}
\providecommand{\spn}{\text{span}}
\providecommand{\Spec}{\text{Spec}\hspace{0.1em}}
\providecommand{\Stab}{\text{Stab}}
\providecommand{\supp}{\text{supp}}
\providecommand{\Syl}{\text{Syl}}
\providecommand{\syl}{\text{syl}}
\providecommand{\Sym}{\text{Sym}}
\providecommand{\Tor}{\text{Tor}}
\providecommand{\Tr}{\text{Tr}}

% BB Sets
\providecommand{\A}{\mathbb{A}}
\providecommand{\C}{\mathbb{C}}
\providecommand{\F}{\mathbb{F}}
\providecommand{\N}{\mathbb{N}}
\providecommand{\P}{\mathbb{P}}
\providecommand{\Q}{\mathbb{Q}}
\providecommand{\R}{\mathbb{R}}
\providecommand{\Z}{\mathbb{Z}}

% Commands
\providecommand{\nsubgp}{\trianglelefteq}
\providecommand{\p}{\mathfrak{p}}
\renewcommand{\H}{\textbf{H}}
\newcommand{\gw}[1]{\left\langle #1 \right\rangle}
\newcommand{\ovl}[1]{\overline{#1}}

\let\minus\smallsetminus
\let\bar\overline
\let\smsh\wedge

\providecommand{\SH}{\mathcal{SH}}


% Colors
\providecommand{\green}[1]{\textcolor{green}{#1}}
\providecommand{\red}[1]{\textcolor{red}{#1}}
\providecommand{\orange}[1]{\textcolor{orange}{#1}}
\providecommand{\green}[1]{\textcolor{green}{#1}}
\providecommand{\blue}[1]{\textcolor{blue}{#1}}
\providecommand{\purple}[1]{\textcolor{purple}{#1}}



% AT commands
\providecommand{\BG}{\text{BG}}
\providecommand{\BO}{\text{BO}}
\providecommand{\BP}{\text{BP}}
\providecommand{\BU}{\text{BU}}
\providecommand{\BSO}{\text{BSO}}
\providecommand{\BSU}{\text{BSU}}
\providecommand{\BGL}{\text{BGL}}
\providecommand{\coeq}{\text{coeq}}
\providecommand{\cof}{\text{cof}}
\providecommand{\cone}{\text{cone}}
\providecommand{\eq}{\text{eq}}
\providecommand{\EU}{\text{EU}}
\providecommand{\Ex}{\text{Ex}}
\providecommand{\Ext}{\text{Ext}}
\providecommand{\Gr}{\text{Gr}}
\providecommand{\Ho}{\text{Ho}}
\providecommand{\hocofib}{\text{hocofib}}
\providecommand{\hocolim}{\text{hocolim}}
\providecommand{\holim}{\text{holim}}
\providecommand{\KGL}{\text{KGL}}
\providecommand{\ko}{\text{ko}}
\providecommand{\KO}{\text{KO}}
\providecommand{\kq}{\text{kq}}
\providecommand{\KQ}{\text{KQ}}
\providecommand{\KR}{\text{KR}}
\providecommand{\ku}{\text{ku}}
\providecommand{\KU}{\text{KU}}
\providecommand{\Lan}{\text{Lan}}
\providecommand{\MGL}{\text{MGL}}
\providecommand{\MO}{\text{MO}}
\providecommand{\MSL}{\text{MSL}}
\providecommand{\MSO}{\text{MSO}}
\providecommand{\MSp}{\text{MSp}}
\providecommand{\MU}{\text{MU}}
\providecommand{\Out}{\text{Out}}
\providecommand{\pre}{\text{pre}}
\providecommand{\Ran}{\text{Ran}}
\providecommand{\RO}{\text{RO}}
\providecommand{\Sing}{\text{Sing}}
\providecommand{\SO}{\text{SO}}
\providecommand{\Spin}{\text{Spin}}
\providecommand{\Sq}{\text{Sq}}
\providecommand{\SU}{\text{SU}}
\providecommand{\Sym}{\text{Sym}}
\providecommand{\TC}{\text{TC}}
\providecommand{\Th}{\text{Th}}
\providecommand{\THH}{\text{THH}}
\providecommand{\TP}{\text{TP}}
\providecommand{\TR}{\text{TR}}
\providecommand{\SH}{\mathcal{SH}}
\providecommand{\Sp}{\textit{Sp}}

% Chromatic
\providecommand{\Prin}{\text{Prin}}
\providecommand{\FGL}{\texttt{FGL}}
\providecommand{\SI}{\texttt{SI}}
\providecommand{\FG}{\text{FG}}
\providecommand{\fg}{\text{fg}}




% Spaces
\providecommand{\CP}{\mathbb{C}\text{P}}
\providecommand{\HP}{\mathbb{H}\text{P}}
\providecommand{\RP}{\mathbb{R}\text{P}}

% Other
\providecommand{\Cech}{\check{C}}
\let\adj\dashv
\let\smashprod\wedge
\RequirePackage{amsmath,amssymb,amsfonts}
\RequirePackage{bbm}


% Categories
\providecommand{\onecat}{\mathbbm{1}}
\providecommand{\twocat}{\mathbbm{2}}
\providecommand{\Alg}{\mathrm{Alg}}
\providecommand{\Ab}{\mathrm{Ab}}
\providecommand{\CAlg}{\mathrm{CAlg}}
\providecommand{\Cat}{\mathrm{Cat}}
\providecommand{\CDGA}{\mathrm{CDGA}}
\providecommand{\CG}{\mathrm{CG}}
\providecommand{\CGWH}{\mathrm{CGWH}}
\providecommand{\Ch}{\mathrm{Ch}}
\providecommand{\CAlg}{\mathrm{CAlg}}
\providecommand{\CMon}{\mathrm{CMon}}
\providecommand{\coAlg}{\mathrm{coAlg}}
\providecommand{\coMod}{\mathrm{coMod}}
\providecommand{\Coh}{\mathrm{Coh}}
\providecommand{\CommRing}{\mathrm{CommRing}}
\providecommand{\Corr}{\mathrm{Corr}}
\providecommand{\CRing}{\mathrm{CRing}}
\providecommand{\CW}{\mathrm{CW}}
\providecommand{\Field}{\mathrm{Field}}
\providecommand{\Fin}{\mathrm{Fin}}
\providecommand{\FinSet}{\mathrm{FinSet}}
\providecommand{\Grp}{\mathrm{Grp}}
\providecommand{\Grpd}{\mathrm{Grpd}}
\providecommand{\Grph}{\mathrm{Grph}}
\providecommand{\Kar}{\mathrm{Kar}}
\providecommand{\Kan}{\mathrm{Kan}}
\providecommand{\Mod}{\mathrm{Mod}}
\providecommand{\lmod}[1]{#1\text{-}\mathrm{Mod}}
\providecommand{\rmod}[1]{\mathrm{Mod}\text{-}#1}
\providecommand{\bimod}[2]{#1\text{-}\mathrm{Mod}\text{-}#2}
\providecommand{\Ouv}{\mathrm{Ouv}}
\providecommand{\Poset}{\mathrm{Poset}}
\providecommand{\PSh}{\mathrm{PSh}}
\providecommand{\PShv}{\mathrm{PShv}}
\providecommand{\qCat}{\mathrm{qCat}}
\providecommand{\QCoh}{\mathrm{QCoh}}
\providecommand{\Rep}{\mathrm{Rep}}
\providecommand{\Ring}{\mathrm{Ring}}
\providecommand{\Set}{\mathrm{Set}}
\providecommand{\SH}{\mathcal{SH}}
\providecommand{\Sh}{\mathrm{Sh}}
\providecommand{\Shv}{\mathrm{Shv}}
\providecommand{\Spectra}{\mathrm{Spectra}}
\providecommand{\sAb}{\text{sAb}}
\providecommand{\sSet}{\mathrm{sSet}}
\providecommand{\Stack}{\mathrm{Stack}}
\providecommand{\Top}{\mathrm{Top}}
\providecommand{\Ring}{\mathrm{Ring}}
\providecommand{\Vect}{\mathrm{Vect}}

% Other
\providecommand{\cyc}{\text{cyc}}
\providecommand{\dg}{\text{dg}}
\providecommand{\gen}{\text{gen}}
\providecommand{\inj}{\text{inj}}
\providecommand{\mor}{\text{mor}}
\providecommand{\Mor}{\text{Mor}}
\providecommand{\ob}{\text{ob}}
\providecommand{\obj}{\text{obj}}
\providecommand{\proj}{\text{proj}}
\providecommand{\Span}{\text{Span}}

\newcommand{\DDelta}{\bm{\Delta}}


% Limits
\providecommand{\llim}{\varprojlim}
\providecommand{\rlim}{\varinjlim}

\RequirePackage{amsmath,amssymb}

% AG commands
\providecommand{\aff}{\text{aff}}
\providecommand{\Ann}{\text{Ann}}
\providecommand{\Alt}{\text{Alt}}
\providecommand{\Bl}{\text{Bl}}
\providecommand{\Br}{\text{Br}}
\providecommand{\ch}{\text{ch}}
\providecommand{\CH}{\text{CH}}
\providecommand{\Cl}{\text{Cl}}
\renewcommand{\div}{\text{div}}
\providecommand{\Div}{\text{Div}}
\providecommand{\Frob}{\text{Frob}}
\providecommand{\Gr}{\text{Gr}}
\providecommand{\Krulldim}{\text{Krulldim}}
\providecommand{\Max}{\text{Max}}
\providecommand{\nil}{\text{nil}}
\providecommand{\Pic}{\text{Pic}}
\providecommand{\Proj}{\text{Proj}\hspace{0.1em}}
\providecommand{\PSh}{\text{PSh}}
\providecommand{\red}{\text{red}}
\providecommand{\SK}{\text{SK}}
\providecommand{\sm}{\text{sm}}
\providecommand{\Sh}{\text{Sh}}
\providecommand{\Spec}{\text{Spec}\hspace{0.1em}}
\providecommand{\Specmax}{\text{Specmax}\hspace{0.1em}}
\providecommand{\Sym}{\text{Sym}}
\providecommand{\td}{\text{td}}
\providecommand{\trdeg}{\textit{tr}.\textit{deg}\hspace{0.1em}}
\providecommand{\Val}{\text{Val}}
\providecommand{\Var}{\text{Var}}
\providecommand{\Zar}{\text{Zar}}

% AG Categories
\providecommand{\Aff}{\texttt{Aff}}
\providecommand{\AffVar}{\texttt{AffVar}}
\providecommand{\Coh}{\texttt{QCoh}}
\providecommand{\QCoh}{\texttt{Coh}}
\providecommand{\Sch}{\texttt{Sch}}
\providecommand{\preVar}[1]{\texttt{preVar}\text{-}#1}
% AG Symbols
\providecommand{\A}{\mathbb{A}}
\providecommand{\Gm}{\mathbb{G}_{\text{m}}}
\providecommand{\m}{\mathfrak{m}}
\renewcommand{\O}{\mathscr{O}}
\providecommand{\p}{\mathfrak{p}}
\renewcommand{\P}{\mathbb{P}}
\providecommand{\q}{\mathfrak{q}}

% AG Arrows
\providecommand{\dashto}{\dashrightarrow}
\providecommand{\dashfrom}{\mathrel{\reflectbox{\ensuremath{\dashrightarrow}}}}

\let\und\underline


